Firenze: Model Evaluation Using Weak Signals

Data labels in the security field are frequently noisy, limited, or biased towards a subset of the population. As a result, commonplace evaluation methods such as accuracy, precision and recall metrics, or analysis of performance curves computed from labeled datasets do not provide sufficient confidence in the real-world performance of a machine learning (ML) model. This has slowed the adoption of machine learning in the field. In the industry today, we rely on domain expertise and lengthy manual evaluation to build this confidence before shipping a new model for security applications. In this paper, we introduce Firenze, a novel framework for comparative evaluation of ML models' performance using domain expertise, encoded into scalable functions called markers. We show that markers computed and combined over select subsets of samples called regions of interest can provide a robust estimate of their real-world performances. Critically, we use statistical hypothesis testing to ensure that observed differences-and therefore conclusions emerging from our framework-are more prominent than that observable from the noise alone. Using simulations and two real-world datasets for malware and domain-name-service reputation detection, we illustrate our approach's effectiveness, limitations, and insights. Taken together, we propose Firenze as a resource for fast, interpretable, and collaborative model development and evaluation by mixed teams of researchers, domain experts, and business owners.

==> sections/DNSReputationTests.tex <==
%\subsection{Comparing Domain Name Reputation Models with K=10,000}\label{tests:10k}

\begin{table}[H]
	\centering
	\caption{Top K test (K=10,000)}
	\label{tab:top10k}
	\resizebox{0.475\textwidth}{!}{%	
		\begin{tabular}{l|r|r|r|c} 
			\textbf{Marker} & \textbf{Avg Marker Score}  & \textbf{Avg Marker Score}  & \textbf{p-value} & \textbf{Result} \\
			& \textbf{Reference Model}  & \textbf{Test Model}  &  &  \\
			\hline
			AbusedDomain	&	0.310569	&	0.294771	&	2.07E-02	&	\color{red}F	\\
			SinkholedDomain	&	0.062194	&	0.020898	&	1.26E-47	&	\color{red}F	\\
			HoneypotDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			DomainPopularity	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			NumberIPs	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			NumberTTLs	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			KnownFutureLabel	&	0.272273	&	0.217278	&	6.88E-19	&\color{red}F	\\
			CombinedMarkerScore	&	0.617138	&	0.516348	&	4.79E-46	&	\color{red}F	\\
		\end{tabular}
	}
\end{table}

\begin{table}[H]
	\centering
	\caption{Bottom K Test (K=10,000)}
	\label{tab:bot10k}
	\resizebox{0.475\textwidth}{!}{%	
		\begin{tabular}{l|r|r|r|c}
			\textbf{Marker} & \textbf{Avg Marker Score}  & \textbf{Avg Marker Score}  & \textbf{p-value} & \textbf{Result} \\
			& \textbf{Reference Model}  & \textbf{Test Model}  &  &  \\
			\hline
			AbusedDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			SinkholedDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			HoneypotDomain	&	0.0001	&	0	&	0.241959	&	\color{YellowOrange}U	\\
			DomainPopularity	&	-0.1875	&	-0.7806	&	0.00E+00	&	\color{green}S	\\
			NumberIPs	&	-0.2614	&	-0.669	&	0.00E+00	&	\color{green}S	\\
			NumberTTLs	&	-0.0631	&	-0.3632	&	0.00E+00	&	\color{green}S	\\
			KnownFutureLabel	&	-0.4275	&	-0.7642	&	0.00E+00	&	\color{green}S	\\
			CombinedMarkerScore	&	-0.5795	&	-0.9835	&	0.00E+00	&	\color{green}S	\\
		\end{tabular}
	}
\end{table}

\begin{table}[H]
	\centering
	\caption{Up-Movers and Down-Movers Test (K=10,000)}
	\label{tab:movers10k}
	\resizebox{0.475\textwidth}{!}{%	
		\begin{tabular}{l|r|r|r|c}
			\textbf{Marker} & \textbf{Avg Marker Score}  & \textbf{Avg Marker Score}  & \textbf{p-value} & \textbf{Result} \\
			& \textbf{Up-Movers}  & \textbf{Down-Movers}  & &  \\
			\hline
			AbusedDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			SinkholedDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			HoneypotDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U	\\
			DomainPopularity	&	-0.0006	&	-0.0038	&	3.44E-06	&	\color{green}S	\\
			NumberIPs	&	0	&	-0.0003	&	8.90E-02	&	\color{YellowOrange}U	\\
			
			NumberTTLs	&	-0.0006	&	-0.004	&	1.35E-06	&	\color{green}S	\\
			KnownFutureLabel	&	0.0033	&	0.0133	&	4.32E-09	&	\color{red}F	\\
			CombinedMarkerScore	&	0.0026	&	0.0074	&	1.06E-02	&	\color{red}F	\\
			
		\end{tabular}
	}
\end{table}

%\subsection{Comparing Domain Name Reputation Models with K=100,000}\label{tests:100k}

\begin{table}[H]
	\centering
	\caption{Top K test (K=100,000)}
	\label{tab:top100k}
	\resizebox{0.475\textwidth}{!}{%
		\begin{tabular}{l|r|r|r|c}
			\textbf{Marker} & \textbf{Avg Marker Score}  & \textbf{Avg Marker Score}  & \textbf{p-value} & \textbf{Result} \\
			& \textbf{Reference Model}  & \textbf{Test Model}  &  &  \\
			\hline
			AbusedDomain	&	0.088239	&	0.063599	&	4.39E-95	&	\color{red}F
			\\
			SinkholedDomain	&	0.237948	&	0.125499	&	0.00E+00	&	\color{red}F
			\\
			HoneypotDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U
			\\
			DomainPopularity	&	-0.00017	&	-0.00014	&	3.45E-01	&	\color{YellowOrange}U
			\\
			NumberIPs	&	0	&	-0.00001	&	2.42E-01	&	\color{YellowOrange}U
			\\
			NumberTTLs	&	-0.00018	&	-0.00014	&	3.11E-01	&	\color{YellowOrange}U
			\\
			KnownFutureLabel	&	0.268607	&	0.235748	&	2.86E-63	&	\color{red}F
			\\
			CombinedMarkerScore	&	0.570214	&	0.405806	&	0.00E+00	&	\color{red}F \\
		\end{tabular}
	}
\end{table}


\begin{table}[H]
	\centering
	\caption{Bottom K Test (K=100,000)}
	\label{tab:bot100k}
	\resizebox{0.475\textwidth}{!}{%
		\begin{tabular}{l|r|r|r|c}
			\textbf{Marker} & \textbf{Avg Marker Score}  & \textbf{Avg Marker Score}  & \textbf{p-value} & \textbf{Result} \\
			& \textbf{Reference Model}  & \textbf{Test Model}  &  &  \\
			\hline
			AbusedDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U
			\\
			SinkholedDomain	&	0	&	0.00001	&	2.42E-01	&	\color{YellowOrange}U
			\\
			HoneypotDomain	&	0.00003	&	0.00002	&	3.61E-01	&	\color{YellowOrange}U
			\\
			DomainPopularity	&	-0.23787	&	-0.49372	&	0.00E+00	&	\color{green}S
			\\
			NumberIPs	&	-0.16872	&	-0.19044	&	6.84E-36	&	\color{green}S
			\\
			NumberTTLs	&	-0.08835	&	-0.22822	&	0.00E+00	&	\color{green}S
			\\
			KnownFutureLabel	&	-0.43925	&	-0.46809	&	1.46E-37	&	\color{green}S
			\\
			CombinedMarkerScore	&	-0.54655	&	-0.67804	&	0.00E+00	&	\color{green}S\\
			
		\end{tabular}
	}
\end{table}


\begin{table}[H]
	\centering
	\caption{Up-Movers and Down-Movers Test (K=100,000)}
	\label{tab:movers100k}
	\resizebox{0.475\textwidth}{!}{%
		\begin{tabular}{l|r|r|r|c}
			\textbf{Marker} & \textbf{Avg Marker Score}  & \textbf{Avg Marker Score}  & \textbf{p-value} & \textbf{Result} \\
			& \textbf{Up-Movers}  & \textbf{Down-Movers}  & &  \\
			\hline
			AbusedDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U
			\\
			SinkholedDomain	&	0	&	0.00002	&	1.47E-01	&	\color{YellowOrange}U
			\\
			HoneypotDomain	&	0	&	0	&	NaN	&	\color{YellowOrange}U
			\\
			DomainPopularity	&	-0.00008	&	-0.00059	&	1.47E-09	&\color{green}S
			\\
			NumberIPs	&	-0.00003	&	-0.00005	&	3.11E-01	&	\color{YellowOrange}U
			\\
			NumberTTLs	&	-0.00006	&	-0.00091	&	2.62E-17	&	\color{green}S
			\\
			KnownFutureLabel	&	0.00048	&	0.00138	&	2.88E-04	&	\color{red}F \\
			CombinedMarkerScore	&	0.00036	&	0.00016	&	2.96E-01	&	\color{YellowOrange}U\\
		\end{tabular}
	}
\end{table}

==> sections/background.tex <==
Cyber Security is a critical area of application of Machine Learning. Unlike most applications of Machine Learning (recommender systems, language translation, computer vision etc), the cost of both a false positive and a false negative is relatively high. A false positive alert may require an analyst to spend hours investigating the activity in question to understand if an attack happened, wasting a scarce resource and lowering trust in the system. Whereas, a false negative may lead to an organization being left open to a ransomware attack, stolen information or any of the numerous negative impacts from the cyber attacks we have seen in recent years and months. Thus the bar that a Machine Learning based system has to meet in a cyber security application is high. 
And while we have seen many studies applying novel combinations of Machine Learning techniques to security problems, we often see that their performance as measured by the mathematical methods of the machine learning domain is not reflected in the operational setting. This is directly seen in the imbalance that exists between extensive academic research published in the area and the rarity of operational deployments of such systems [reference paxson paper].

So why is it that ML algorithms that perform well on traditional data science metrics like PR curve, precision and recall etc don’t do well in operational settings? We give 4 reasons here.

\begin{itemize}
	\item Real world data distributions are different and more complex than what is represented in the training data: The most critical ingredient in an ML system is the data. [reference Data centric machine learning]. Its closeness to the real intended environment of operation for the model is a critical factor in the model’s performance. Let us consider an example application in Malicious domain classification. 
	\begin{itemize}
		\item The universe is much more complex compared to the training data: A reasonably large training dataset may have X million malicious and Y million benign domains [insert real data from Mithra or other paper reference]. But a large enterprise like Amazon sees upwards of Z billion domains per day, out which W million are seen for the first time [insert right numbers from Mithra/Amazon]. Millions of new domains are registered everyday, new tlds are created, some of these are for purely malicious reasons, the type of maliciousness may change over time, some are benign but get hacked or otherwise tricked into being used for malicious purposes and others still are parked or sinkholed so the characteristics of their traffic (and their label) keep evolving. This complexity is hard to represent in training data that is at best 1/10th of the size of daily traffic, realistically much smaller.
		\item Concept drift: the characteristics of malicious domains change over time as attackers eveolve their tactics. This is hard to track and represent adequately in training data.
	\end{itemize}
	\item Labels are noisy, sparse or absent: Compared to the size of our universe, the amount of labeled data we have is small for most security applications. For some applications like detecting APT attacks, the data is mostly not available outside a few select companies. This is often due to the sensitive nature of the data. 
	\item Reliable ground truth is absent for evaluation: Out of the Z billion domains seen every day, event dedicated security teams will be able to provide ground truth for only a small fraction of the entities [insert same number from above]. 
	\item Feedback is infrequent and imperfect: Most users of these algorithms do not provide frequent feedback. Only egregious FPs or FNs elicit questions or critisicms. The decisions that are correct, or left uninvestigated (most of the decisions) don’t.
\end{itemize}

Yet, machine learning systems are an important component of defense in depth because security skills are scarce, their demand is growing and ML can help defenders scale. So today, to estimate the real-world performance of an ML system we conduct a manual evaluation of its findings by domain experts. It is common to run a model in “shadow mode” or “replay mode” and have Security Researchers manually examine clusters of results that seems like outliers or otherwise “interesting” based on their experience or maybe in comparison to a reference system. They then certify that a model is free from obvious FPs and FNs, which then allows the deployment of the model. 

There are several limitations to this approach. (1) It takes a long time to conduct this analysis. It may involve a researcher investigating several clusters of unknown activity to determine whether the model was right or wrong, and this is a labor intensive process. (2) It uses security skills that are already in short supply. And (3) it negatively impacts on the ability to innovate and iterate quickly on ML techniques since every iteration requires this manual analysis to determine real efficacy. 



==> sections/firenze1.tex <==
TODO Questions:
-- Do we need to have a bound on markers (we should test the simulation with oracle and feed labels being the same.)


\subsection{Markers}
A marker is a weak signal that is cheaply obtained and is associated with the maliciousness or benignity of a sample, instance, or event. The weak signal can come from multiple sources, patterns, heuristics and external knowledge bases as long as they are based on domain expertise. 
\subsubsection{Marker Quality}
Past works in weak supervision have made assumptions about the quality of the weak signal being used but left out methods of verification of those assumptions. e.g. in \cite{ratner2017data} weak signals are called labeling functions. It makes the following assumptions— for a labeling function, $\beta$ is the probability of it labeling an object and $\alpha$ is the probability that it labels the object correctly. The paper assumes that 0.3 < $\beta$ < 0.5 and 0.8 < $\alpha$ < 0.9 and that the classes are balanced. i.e. each class has a probability of 0.5. 
One of the key values of our work is to combine these weak supervision with domain expertise, which we use here to estimate whether our assumptions are met. To ensure the markers are of adequate quality, we will be measuring the following parameters. 
\begin{itemize}
	\item Coverage $\beta = \frac {Number of times Marker votes} {Number of Samples}$
	\item Conditional Accuracy $\alpha = \frac {Number of times Marker is right} {Number of times Marker votes}$
\end{itemize}
Based on the simulations, we know that we need we can tolerate extremely low coverage if we have good accuracy. We will be using only signals that have $\alpha$ >0.6. We choose this level because the simulations show that this is the minimum required level to ensure the right outcome for our equations. They also show that at this level, the significance test is robust to provide the right outcome, or an undetermined result if the coverage is too low for a given marker. And this holds for different class balance settings, different sizes of “locally interesting regions” and different magnitudes of difference in model performance on known data.
Since we are combining the markers using majority voting, we expect the combined Marker Score to meet or exceed this bar (proof needed?). {\bf \color{red} Ali: Are we not doing the summation anymore?--Doesn't make difference in the hypothesis tests part though.}
A key advantage of this approach is that the availability of individual markers and performance of a model relative to them gives explainability to the fitness of the model— this is a key factor, since it help build trust for machine learning in the security community and moves away from treating it as a black box.
For future research, we aim to explore the value of combining the markers using a generative model to improve the quality of the combined marker score. Existing research does show that for < 10 signals, majority voting outperforms generative models, so we are confident in the value of the current approach \cite{Snorkel2017}.


\subsection{Score Spectra of Two Models}
Most machine learning models generate a ``score" value vector $\mathbf{p}_{i} \in \mathbb{R}^{\|\mathcal{C}\|}$ for each sample $i$, which reflect the ``confidence" or the ``probability" of  the $i$th sample belonging to each of $\|\mathcal{C}\|$ possible classes. While these values are usually non-negative and are normalized to add up to $1.0$--with a degree of freedom equal to $\|\mathcal{C}\|-1$, they can also be the raw score output of a model such as logit values in the last layer of a neural network, or the reconstruction error of an auto-encoder. Our goal is to design a pairwise model-comparison framework for both supervised (e.g.,~classification of malicious vs.~benign domain names) and unsupervised score-based model such as anomaly detection using auto-encoders.

In this subsection, first we explain how we try to have an apple-to-apple comparison of generated scores accross two different models, where we argue that a rank transformation is the appropriate choice for avoiding complex cross-model score calibrations. Then, we explain our choices for interesting regions of score-based rank spectra for compraing two models.

{\bf Score vs.~rank.} For many machine learning models, by using transformations such as {\bf SoftMax}, the raw scores of a sample can be mapped to equivalent probabilistic measures, yet for models like auto-encoders, such a transformation either does not exist or the normalization is expensive or nontrivial. On the other hand, although the model scores are internally meaningful in each model itself, uncalibrated scores that are generated by two models under different parameterization or data settings do not necessarily reflect the same comparable absolute values. For example, model {\it A} might score a set of samples in Range $[0, 0.8]$, where model {\it B} scores the same set of samples in range of $[0, 0.9]$. Fair comparison of such two models cannot be done without proper calibrations. When the scores do not have a predefined range, interpretation and model comparisons become even more challenging. At the same time, if we sort the samples by their scores in each model, the ranking of that sample will be comparable with rankings generated by the other models. 

In this work, we exploit the rank of a sample by a model based on incremental ordering of score values. By using ranks, we bypass the problem of score calibration. As an example, in the binary classification case for malicious vs. benign samples, the ordeing generated by each models' scores will reflect the relative confidence of the model for maliciousness of a sample. Now when comparing models {\it A} and {\it B}, we only compare the correctness of this model-internal relative confidence, without dealing with potentially non-linear mapping from one score set to another one.

{\bf Regions of interest.} In security applications as a general rule, a better model is the model  that makes more clear separation between malicious and benign samples.  The goal is often to detect confidently benign or  confidently malicious samples.  However, an improvement in the model might not change the most confident predictions on the extreme of the score spectra of the two models. But, a better model migh change the rank of samples in the right direction. Therefore, we propose to perform separate model comparisons on the following three ``regions of interest":

\begin{itemize}
	\item Top ranked: We need the model to produce high quality list of malicious domains names with {\bf  few or no false positives.} A better model  should contain more high-raked malicious.
	\item Low-rankedl: The better model assign lowest ranks to most benign samples.
	\item Movers: A new model is better than an old model, if  in aggregation the direction of movement of malicious is towards higher ranks, and benign samples are ranked lower compared to the previous model.
\end{itemize}

The first two bullet points refer to most clearly separated sets of samples by each model, but we need the scores in the gray area (not the lowest or the highest scored  groups of samples) be meaningful as well. This quality is captured by the third bullet point. If the new, which is to be proven better has ranked a sample significantly higher or lower — not necessarily changing the prediction decision — then that rank change should be aligned with our domain expert expectations.  We don’t expect the ranks to be exactly the same across the two models. Therefore, we propose to compare top movers. Top up-movers should be significantly more malicious than top down-movers for the new model to be better.



\subsection{Hypothesis Based Tests}

A marker is a weak indicator that is associated with maliciousness of a sample. For each application, we design a number of markers using our domain expertise—the more markers are designed the better.  Markers are used for measuring maliciousness of individual or sets of samples. We design $M$ marker functions $\{m_1, \dots, m_M\}$, where $m_j(s) $ indicates if the $j$’s marker is observed for Sample $s$.  We assume $m_j(s)$  is zero or one for now, however, continuous values will also work similarly in our proposed framework. In particular, $m_j(s)$ could also reflect the importance/effectiveness of Marker $j$ in capturing if  Sample $s$ is malicious or benign. We use a negative valued  $m_j(s) $ function to reflect the benign property.

The main intuition behind how markers can be used is *Marker-scoring a sample:* For each  sample $s_i$, we define:

\begin{align}
	z_i = \sum_{j=1}^Mm_j(s_i)  
\end{align}

The higher the value of  $z_i$ is the more malicious Sample $s_i$ is expected to be.

We propose to perform a paired T-test for each region of interest that we introduced in the previous subsection.

{\bf Hypothesis Testing.} For each statistical test in the following, we want to see if new Model C or old Model E have ranked the samples such that the more malicious samples have higher ranks, and the most benign (least malicious) samples are low-ranked. In other words, we would like to test if Model C’s high-ranked samples have significantly higher *marker-scores* on average compared to Model E’s. On the other hand, for the lower end of models’ score spectrums, model C is better when the average of marker-scores on its low-ranked samples is significantly lower than model E’s. 

\eat{Null hypotheses: We form a null hypothesis for each scenario. In each test, if the null hypothesis (H0​) ``is not very unlikely (or equivalently if H0​ is a little (or very ) likely"), then the existing model E  wins the test. (Otherwise, H0​ ``is not likely", then we accept Model C is the winner.)
Alternate hypotheses: An alternate hypothesis (Ha​) is the inverse of the null hypothesis, which implies the Model C is better than Model E. Model C wins a test if the null hypothesis ``is very unlikely", i.e., probability of H0​ is less than some value alpha (e.g., α=0.05). 
Probability distribution of null hypothesis:  To determine how likely the null hypothesis is, we should use the right probability distribution based on our random variables which are the marker-scores for each sample. The major quantity that we use in the tests is the sum of triggered marker functions for each sample. If the marker values are 0 and 1, then a binomial distribution is the right choice, especially when M (the number of markers) is a small number. However, in our final step of the test we always use the average of marker-scores in a two-sample (https://en.wikipedia.org/wiki/Two-sample_hypothesis_testing) or paired (https://en.wikipedia.org/wiki/Paired_difference_test) statistical test scenario. Therefore, as our sample size is usually large the averages values can be approximated by a normal or a t-distribution. (I.e., average of marker-scores from each of the models in a two-sample setting, or the average of the difference between marker-scores for the same samples in a paired setting can be approximated by a normal or a t-distribution.) Since its possible to observe fat-tails in our data (specially when our sampling is biased, e.g., from the extreme ends of the spectrum), we will use a t-distribution as the probabilistic model for the null hypothesis.
Two-sample t-test: In the following tests, some times we choose high or low-ranked samples based on each models outcome, where potentially different samples will be chosen for each one of the models C and E. (Although some shared samples could be chosen from both model score sets, e.g., the top K scored samples by both models can have overlaps. But, the overlap will not impact our analysis negatively.) For such scenarios, we will apply a two-sample t-test to the average of marker-scores for each chosen subset of samples. While the random variables are based on the same marker-scores, we still don’t know if the sampling bias would result in different sample variances or not. Therefore, we propose to use a Welch test (two-sample t-test assuming different variances),  However, for each test/application, it makes sense to compare the variances first on biased subsets, and if they are in the same range the use equal variance two-sample t-test.
Algorithm two-sample t-test:
Receive values (marker-scores) for each sample:   ZT​={zi1​​,…,ziLT​​​} and ZR​={zi1​​,…,ziLR​​​} 
H0​:  Values of   ZT​ are larger on average than the values of ZR​ 
Compute the means values in each set: zˉT​=∣ZT​∣1​∑z∈ZT​​z, zˉR​=∣ZR​∣1​∑z∈ZR​​z
Compute the sample variances of values in each set: VT​=∣ZT​∣−11​∑z∈ZT​​(z−zˉT​)2,  VR​=∣ZR​∣−11​∑z∈ZR​​(z−zˉR​)2
Compute the t-statistics (assuming unequal variances): t=VT​/∣ZT​∣+VR​/∣ZR​∣​zˉT​−zˉR​​
Compute  the one sided p-value using the t-distribution with degree of freedom equal to min(∣ZT​∣,∣ZR​∣)
if p-value < 0.05 reject the null hypothesis.
paired t-test: For some of test rounds, we would like to know how models C and E have scored the same samples differently. For these rounds we use paired t-test.
Algorithm paired t-test:
Receive measure differences for each sample:   D={d1​,…,dL​} 
H0​:  Average of D≤0 
Compute the average of values: dˉ=∣D∣1​∑d∈D​d
Compute the sample variance: s=∣D∣−11​∑d∈D​(d−dˉ)2
Compute the t-statistics: t=Ls​​dˉ​
Compute  the one sided p-value using t-distribution
if p-value < 0.05 reject the null hypothesis.}


\subsection{Decision Criteria}
Business decicion



==> sections/future.tex <==
%We adopt the following relational graph convolutional network to identify the malicious domains. Assume we have in total $K$ relations, where one of the relation denotes connecting to the node itself (``self-loop'') and denote its index as $s$. Each relation here denotes a directed edge between two partites in a bi-partite graph. Since our graph is assumed to be undirected, for each bi-partite graph, we will have two relations corresponding to edge and the inverse edge. 
% $E_1, \ldots, E_K$ (1: ec2-sub, 2:ip:sub, 3:self)
%$h_i^{0} = x_i$, where $x_i$ is the node feature. Based on the representation in layer $l$, the representation at layer $l+1$ can be obtained as:
%$$h_i^{(l+1)} = f(\sum_{k=1,k\neq s}^K \sum_{j\in\mathcal{N}^{k}(i)\backslash i} \frac{1}{c_{ik} } w_{l, k} h_{j}^{l} + w_{l,s}h_{i}^{l}),$$
%where $c_{ik} = 1$ is the normalizing factor and we adopt the Edge normalization for our tasks.  $f(x)$ is the activation function and we use ReLU function for our tasks.  

We adopt the following relational graph convolutional network to identify the malicious domains. Assume we have in total $K$ relations, where one of the relation denotes connecting to the node itself (``self-loop'') and denote its index as $s$. Each relation here denotes a directed edge between two partites in a bi-partite graph. Since our graph is assumed to be undirected, for each bi-partite graph, we will have two relations corresponding to edge and the inverse edge. 
% $E_1, \ldots, E_K$ (1: ec2-sub, 2:ip:sub, 3:self)
$h_i^{0} = x_i$, where $x_i$ is the node feature. Based on the representation in layer $l$, the representation at layer $l+1$ can be obtained as:
$$h_i^{(l+1)} = \sigma \big(\sum_{k=1}^K 
\frac{1}{|\mathcal{N}^{k}(i)|+1}(\sum_{j\in\mathcal{N}^{k}(i)} \frac{1}{c_{ik} } w_{l, k} h_{j}^{l} + w_{l,0}h_{i}^{l})\big),$$
where $c_{ik}$ is the normalizing factor and in our current experiment, we set $c_{ik}=1$, and will explore more customized normalizing factors. $\sigma(x)$ is the activation function and we use ReLU function for our experiments. $\mathcal{N}^{k}(i)$ denotes the neighbors of node $i$ in relation $k$, but excludes the node $i$ itself. 



\subsection {Ensemble Method}
TODO: What we did. Theoretical guarantees?



\subsection {Potential Track: Learning to Ignore}


$\text{msg}_i^l= \begin{cases}
(h_i^l, 0)& r(x_i) \leq 0.5 \quad \text{Accepted} \\ 
(\text{No Embedding}, g_i^l)& r(x_i) > 0.5 \quad \text{Deffered} 
\end{cases}$ -- penalty for misclassification

$\text{msg}_i^l= \begin{cases}
(h_i^l, 0)& r(x_i) \leq 0.5 \quad \text{Accepted} \\ 
(\mathbf{0}, g_i^l)& r(x_i) > 0.5 \quad \text{Deffered} 
\end{cases}$ -- penalty for misclassification

$\text{msg}_i^l= (h_i^l, g_i^l)$

$h_i^l  =  h_i^l \mathbb{I}(r(x_i) \leq 0.5)$


$g_i^l = g\left(r(x_i), \sum_{j\in \mathcal{N}(i)} r(x_j)\right)~ \mathbb{I}(r(x_i) > 0.5)$ -- penalty for ignorance

%x_i^l, g_i^l --> message

$g_i^l = r(x_i) + \frac{\sum_{j\in \mathcal{N}(i)} \mathbb{I}(r(x_i) > 0.5)}{|\mathcal{N}(i)| - \sum_{j\in \mathcal{N}(i)} \mathbb{I}(r(x_i) \leq 0.5)}$

$g_i^l = r(x_i) + \frac{\sum_{j\in \mathcal{N}(i)} r(x_j)~\mathbb{I}(r(x_i) > 0.5)}{|\mathcal{N}(i)| - \sum_{j\in \mathcal{N}(i)} r(x_j)~\mathbb{I}(r(x_i) \leq 0.5)}$

$g_i^l = r(x_i) + \frac{\sum_{j\in \mathcal{N}(i)} r(x_j))}{|\mathcal{N}(i)| - \sum_{j\in \mathcal{N}(i)} r(x_j))}$

$g_i^l = r(x_i) + \frac{\sum_{j\in \mathcal{N}(i)} r(x_j))}{|\mathcal{N}(i)| - \sum_{j\in \mathcal{N}(i)} r(x_j))}$

$l(f(x_i), y_i)~\mathbb{I}(r(x_i) \leq 0.5)$ -- penalty for misclassification

$l(f(x_i), y_i)~\mathbb{I}(r(x_i) \leq 0.5) + \lambda g(r(x_i), \sum_{j\in \mathcal{N}(i)} r(x_j))~ \mathbb{I}(r(x_i) > 0.5)$ 

$l(h_i^{L}, y_i) + \lambda \sum_{l=1}^{L} g_i^{l}$ 

$l(f(x_i), y_i) * g(r(x_i), \sum_{j\in \mathcal{N}(i)} r(x_j))$ 




Below are some loss functions we discussed before the presentation.
$g_i^l = r(x_i) + \frac{\sum_{j\in \mathcal{N}(i)} r(x_j))}{|\mathcal{N}(i)| - \sum_{j\in \mathcal{N}(i)} r(x_j))}$

$g_i^l = r(x_i) + \frac{\sum_{j\in \mathcal{N}(i)} r(x_j))}{|\mathcal{N}(i)}$

$g_i^l = (1-\alpha )r(x_i) + \alpha \frac{\sum_{j\in \mathcal{N}(i)} r(x_j))}{|\mathcal{N}(i)}$

$h_i^l  =  h_i^l ~ \mathbb{I}(g_i^l \leq 0.5)\quad \forall ~~ i \in \{\text{layers and partites}\} - \{\text{last layer}\}$ 

$g_i^l = (1-\alpha )r(x_i) + \alpha \frac{\sum_{j\in \mathcal{N}(i)} g_j^{(l-1)}}{|\mathcal{N}(i)}\quad\forall ~~ i \in \{\text{layers and partites} - \{\text{last layer}\}, ~ \alpha\in [0, 1]$

$g_i^l = g\left(r(x_i), \sum_{j\in } g_j^{(l-1)}, |\mathcal{N}(i)|\right)$

$Loss(w, \theta) = \mathbb{I}(g_i^L \leq .5)l(h_i^{L}, y_i) + \lambda \mathbb{I}(g_i^L >.5)  g_i^L \quad \forall ~~ i \in \{\text{last layer}\}$

$Loss(w, \theta) = \mathbb{I}(g_i^L \leq .5)l(h_i^{L}, y_i) + \lambda \mathbb{I}(g_i^L >.5)  g_i^L \quad \forall ~~ i \in \{\text{last layer}\}$

$Loss(w, \theta) = \mathbb{I}(g_i^L \leq .5)l(h_i^{L}, y_i) + \lambda \mathbb{I}(g_i^L >.5)  l_{exp}(h_i^{L}, y_i) \quad \forall ~~ i \in \{\text{last layer}\}$

$Loss(w, \theta) = \mathbb{I}(g_i^L \leq .5)l(h_i^{L}, y_i) + \lambda \mathbb{I}(g_i^L >.5) \left(g_i^L + \sum_{k \in \text{Expert Types}} l_{k}(h_i^{L}, y_i)\right) \quad \forall ~~ i \in \{\text{last layer}\}$



==> sections/hypothesis_tests.tex <==
{\bf General question: How to decide if a current new model (Model C) is better than the  existing old model (Model E)?}

When, we build ML models to detect malicious entities or activities for various security use cases, we regularly encounter a major issue. We almost always lack reliable source of labelled ground-truth data. Without such reliable ground-truth data, how do we evaluate new ML models we build and verify that they work better than existing methods in production? In this document, we lay out a possible solution to this problem. *The proposed framework is an attempt to systematically ingest domain expertise and decide whether the new model is better than the existing solution in production in a principled way.*

In absence of enough reliable ground truth data, existing methods for comparing the performance of two binary classifiers require a decent reference classifier. The reference classifier should perform better than random one on the same use case in question. These methods statistically reason whether classifier C is better than classifier E based on how often they agree with the reference classifier and disagree with each other. In our use cases, however, we often have a severe class imbalance — overwhelming majority of the data points belong to one class — and therefore we don’t have a decent reference classifier.

Without such reference classifier, the only thing we can do is to accumulate bits and pieces of evidence and slowly build the case that classifier C is better than classifier E. 

*Score vs. rank:* Models C and E might have different natures (e.g., one is a random forest and the other one is a deep model) or might have been trained under different circumstances. Therefore, we cannot assume that probability scores generated ** by the two models be comparable with each other directly. However, the scores are internally meaningful in each model itself. That means if we sort the samples (domains) by their scores in each model, the ranking of that sample will be comparable with rankings generated by the other models.

*Application-specific question:* 
*Which scored sample should vitally  be classified correctly?*
*Short Answer: All samples!* But we have a few potential scenarios. For example for Mithra’s use-cases:


* *Scenario 1: Top-malicious-scored List. 
    
    *We need the model to produce high quality list of malicious domains names with *very few or no False Positives.* 
    * *Requirement*: High ranked samples according to the better model should be *more malicious*.
    * Top-K samples should show more prominent signs of malicious behavior collectively. *[REQ1]*



* *Scenario 2: Top-benign-scored List. 
    
    *We need to produce a list of benign domains, with *very few or no False Negatives.*
    * *Requirement*: Low ranked samples according to the better model should be *more benign* .
    * Bottom-K samples should show more prominent signs of benign behavior collectively. *[REQ2]*



* *Scenario 3*: *Gray area risk evaluation/minimization. Cleaner Trustable/Suspicious Regions.
    
    *We need the scores in the gray area (not the lowest or the highest scored  groups of samples) be meaningful as well. This means if model C has ranked a sample significantly higher or lower — not necessarily changing the prediction decision — then that rank change should be aligned with our domain expert expectations. 
    * *Requirement:* Big movers should have moved in the correct direction collectively.
    * *Up-Movers* should be more malicious samples and *Down-Movers* should be more benign.
    * We don’t expect the ranks to be exactly the same across two models. However, when we compare top-K big movers (up or down); *Up-Movers* should be significantly more malicious than top *Down-Movers* for model C to be better. *[REQ3]*




{\bf Solution recap.} Weak Markers for Comparison: A marker is a weak indicator that is associated with maliciousness of a sample. For each application, we design a number of markers using our domain expertise—the more markers are designed the better.  

Markers are used for measuring maliciousness of individual or sets of samples. We design $M$ marker functions $\{m_1, \ldots, m_M\}$, where $m_j(s)$ indicates if $j$'s  marker is observed for Sample s.  ( We assume $m_j(s)$  is zero or one for now, however, continuous values will also work similarly in our proposed framework. In particular, $m_j(s)$  could also reflect the importance/effectiveness of Marker j in capturing if  Sample s is malicious or benign. We use a negative valued  $m_j(s)$  function to reflect the benign property.)  


The main intuition behind how markers can be used is *Marker-scoring a sample:

For each  sample $s_i$, we define
\begin{align}
	z_i = \sum_{j=1}^Mm_j(s_i)
\end{align}

The higher the value of  $z_i$ is the more malicious Sample $s_i$ is expected to be.

Hypothesis Testing: We compare Model C (current test model) against Model E (existing reference model) , by comparing marker score average on high-scored domains, low-score domains based on each model, as well as comparing the marker score between the samples whose score ranks have  largely changed in Model C compared to their score rank based on Model E.   

\begin{itemize}
	\item {\bf  [REQ1] Test 1: Comparing top-K domains based on models C and E.}
	Model C is better than Model E if the average of marker scores of top-K high-scored domains in Model C is *larger* than the average top-K high markers-scored domains by model E.  Null-hypothesis: The averages of marker-scores for both of the two groups are equal.
	\item {\bf  [REQ2] Test 2: Comparing bottom-K domains based on models C and E.}
	Model C is better than Model E if the average of marker scores of bottom-K low-scored domains in Model C is *smaller* than the average bottom-K low-scored domains by model E.  Null-hypothesis: The averages of the two groups are equal.
	\item {\bf  [REQ3] Test 3:Comparing top-K big movers based on models C and E.}
	Model C is better than Model E, if the average of marker scores of *top-K Up-Movers* is *larger* than the average *top-K Down-Movers* . Null-hypothesis: The averages of the two groups are equal. samples with ascended ranks in Model C should have higher average of marker scores of the one with descended ranks.
	* *Decision:* Depending on the application we might need Model C to be better in a specific test only. For example, for providing suspicious malicious domains, it might suffice that Test 1 has to pass. For generating a benign list of domains, Test 3 needs to pass. As a general rule, we can assume Model C is better if it’s better based on the majority of the tests (2 out of 3.) For a conservative decision, we will accept Model C is better if it’s better in all three tests.
\end{itemize}

==> sections/intro_old.tex <==
Reliable ground-truth labels are often not available in information security. Without such labels, how can we determine whether a newly developed machine learning model would perform better than existing methods if deployed in production? In this work, we consider this fundamental yet common problem, which is arguably the biggest reason why machine learning has suffered slower adoption in information security as opposed to other domains such as computer vision and natural language processing. After all, one needs to demonstrate the additional security value provided by a new ML model in order to make a case for it to replace existing methods. In this work, we aim to automate model evaluation by incorporating domain expertise in a scalable way without requiring ground-truth labels. We believe that such ability to quickly compare ML models would significantly accelerate the iterative development process of machine learning models and hence prompt their adoption in information security.



Obtaining labelled data for machine learning is not trivial on its own, however, it is especially challenging in information security. For example, in computer vision, large number of images can be labelled through crowdsourcing campaigns \cite{mechanical turk} in order to build and evaluate object recognition models. A similar approach can be used to annotate large volumes of text for various natural language processing use cases. While this strategy works well in such natural domains, where being a human is enough to expertly carry out data labeling tasks, it falls short in other domains where domain expertise require years of training and experience. In those type of specific domains, such as information security, data labeling requires painstaking and lengthy investigations, that can only be carried out by a small group of professionals, and hence cannot be easily scaled up through crowdsourcing.

Despite all these challenges, there may be limited set of labeled data available in some rare situations. For example, a list of malicious and benign domain names obtained from third party threat intelligence providers can be used to train and evaluate a  malicious domain classification model. However, the amount of labeled data is often too small compared to the size of the overall population and hence cannot faithfully capture the underlying data distribution. Therefore, any traditional accuracy metric, such as precision and recall, obtained from such test dataset conveys little information regarding how the model would perform on billions of unlabelled domain names it has to score each day in production. In fact, it is not uncommon for a model to yield unreasonably high number of false positives in production, thereby rendering itself impractical, despite achieving near perfect precision and recall scores on labelled test data. Furthermore, any collected labeled data is at a higher risk being obsolete in information security, since adversaries frequently change tactics and move targets, essentially causing a severe concept drift. 


%Presence of an intelligent adversary poses another unique challenge for reliable ground-truth labels in information security. More specifically, ever-evolving adversaries significantly accelerate concept drift as they frequently change tactics and move targets. Therefore, even if in cases a limited set of reliable labeled data available in some rare cases, it is usually inaccurate or outdated representation of the underlying real data distribution. Hence, traditional accuracy metrics, such as precision and recall, computed using such limited labels for a trained model are far from sufficient to signify its actual performance on real world data in production. For example, one can train and evaluate a malicious domain name classifier using a set of malicious and benign domain names obtained from third party threat intelligence providers. Such test accuracy results, however, would convey little information regarding how the model would perform on billions of unlabelled domain names it has to score each day in production. In fact, it is not uncommon for a model, which achieves near perfect precision and recall scores on labelled test data, to yield unreasonably high number of false positives in production, thereby rendering itself impractical.


In the absence of reliable ground-truth data, demonstrating a security value of a machine learning model often comes down to domain experts manually investigating results to build confidence in the new model in question. For example, a security domain expert investigating a new malicious domain name detection model would need to examine numerous domain names flagged malicious by the model in order to verify whether the model performance is acceptable. This process is laborious and slow. It is also expensive since it can only be performed by highly-trained domain experts whose attention is precious and schedules are busy. Furthermore, despite all the effort, this process does not yield any objective measure of accuracy, thereby making it very hard to compare newly developed ML models with existing methods. As a result, developing, deploying and iteratively improving new ML models for information security applications is extremely slow. A fast and simple method to objectively compare a newly developed model with an existing method would significantly accelerate this process of iterative improvement.


In this work we aim to address this issue by automating such manual investigation processes. More specifically, we propose a novel framework which automatically incorporates domain expertise into model evaluation process and objectively determines whether a given ML model performs better than an existing method. We achieve this by first encoding domain expertise as a set of binary rules, called markers. These markers are weak indicators of maliciousness or benignity for data points in a given use case. They collectively represent what domain experts look for to see during manual investigation process in data points that are deemed malicious or benign by the ML model. Once encoded as rules, these markers can automatically be applied to unlabelled test data at scale to automatically reason about the comparative accuracy of a given ML model with respect to existing methods. Essentially, we can verify the performance of a new ML model is better than en existing method by checking how much higher and lower it is able rank data points associated with malicious and benign markers respectively compared to the existing method. Furthermore, thanks to binary construct of these markers, we can also make statistically significance arguments via hypothesis testing by constructing appropriate null-hypothesis assumptions.


The efficacy of our proposed method hinges on the quality of markers designed by domain experts. Naturally, the higher quality the markers are the more reliable our conclusion will be. However, recall that we are not trying to estimate the accuracy of a given model but we are simply interested in the binary question of whether a new ML model performs better than an existing method on a given unlabelled test dataset. We show that our method can reliably answer this binary question by using only a small number of weak markers which need to be slightly better than random guesses. In the remaining of this paper, we demonstrate using a synthetic dataset that how even a single marker can be used to make reliable conclusions. We also apply our method in two real-world use cases malicious domain detection. {\color{red} Need some stitching to the rest of the paper here}


In this work we make the following contributions:

\begin{itemize}
\item Introduce markers which encode domain expertise as a set of rules
\item Develop a series of statistical tests to objectively compare a given pair of machine learning models
\item Demonstrate the efficacy of the approach using synthetic data set and real-world 
\end{itemize}

The rest of the paper is organized as follows; In Section 2 we present.....




==> sections/majorityvotingproof.tex <==
\eat{The following theorems prove that by using the majority voting mechanism in Eq.~\ref{eq:majorityvoting}, a collection of markers with accuracies ($\alpha$) that are better than random increase collective accuracy and coverage that are larger than individual markers. }

First, we assume all markers have the same probability of being correct. Theorem \ref{thm:binom}, proves that given $k$ such markers, where each of them has equal probability of  correctly predicting the true, unobservable label $y_i$. Then, the majority voting performs more accurately than any single marker in the set. 


\begin{theorem} 
	\label{thm:binom}
	Let  $z =  \underset{v\in \{-1, 1\}}{\arg\max}~~ \sum_{j=1}^k1(m_j(s)=v)$ be the majority vote for the label of Sample $s$. If all markers vote "independently" with $\alpha_j=\alpha > .5$  ($\alpha$ being a constant for all $j$'s), then
	\begin{align}
		p(z  = y_s) \geq \alpha
	\end{align}
	where $y_s$ indicates the true label of sample $s$.
\end{theorem}


\begin{proof}
	Let $x=\sum_{j=1}^k1(m_j(s)=y_s)$ be the total number of correct votes for Sample $s$. Since individual markers vote independently, each marker can be seen as an independent Bernoulli random variables with probability of success $=\alpha$. Therefore, sum of such random variables will have a binomial distribution with probability mass function $p(x) = \binom{k}{x} \alpha^x (1-\alpha)^{k-x}$. We are interested in probability that $x > k/2$, which means the majority of markers have voted correctly. In particular 
	\begin{align}
		p(x > k/2) = \sum_{n = \lfloor k/2 \rfloor + 1}^k \binom{k}{n} \alpha^n (1-\alpha)^{k-n}
	\end{align}
	This reduces the theorem to Condorcet's Jury Theorem \cite{condorcet1785essai, austen1996information}, where by induction, we can show that for odd values of $n$ for all values of $\alpha>.5$, we will have $ p(x > k/2)  \geq \alpha $.
\end{proof}

Figure \ref{fig:majority_voting_all} (a) shows how majority voting with different number of voting markers and different values of $\alpha$ can produce a higher quality predictions, compared to the labels generated by one marker only. We also observe that adding more markers with the same accuracy, improves the overall performance of majority voting.  

\eat{\begin{figure}[H]
		\centering
		\includegraphics[width=.7\textwidth]{./figures/marker_comb_majority_voting.pdf}
		\caption{{\bf Majority Voting.} Varying the value of $\alpha$, we observe that with larger number of active markers, the probability of correct prediction increases. A combined set of markers always outperform a single marker. }
		\label{fig:majority_voting_fixed_alpha}
	\end{figure}
}

%\begin{figure}
%	\centering
%	\begin{subfigure}[b]{0.5\textwidth}            
%		\includegraphics[width=\textwidth]{./figures/marker_comb_majority_voting.pdf}
%		\caption{ Majority Voting}
%		\label{fig:majority_voting_fixed_alpha}
%	\end{subfigure}%
%	%add desired spacing between images, e. g. ~, \quad, \qquad etc.
%	%(or a blank line to force the subfigure onto a new line)
%	\begin{subfigure}[b]{0.5\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{./figures/adding_stronger_marker_all_better_than_random.pdf}
%		\caption{Varying $\alpha'$}
%		\label{fig:stronger_marker}
%	\end{subfigure}

\begin{figure}
	\centering
	\includegraphics[width=0.45\textwidth]{./figures/marker_comb_majority_voting.pdf}
	\includegraphics[width=0.45\textwidth]{./figures/adding_stronger_marker_all_better_than_random.pdf}
	\caption{{\bf (a)} Varying the value of $\alpha$, we observe that with larger number of active markers, the probability of correct prediction increases. A combined set of markers always outperform a single marker. {\bf (b)} Given $n-1$ markers with accuracies equal to $\alpha$, we add the $n$th marker with accuracy with accuracy $\alpha'$. We observe with more markers (e.g., 10),  adding a stronger or weaker marker will have a negligible impact, but with fewer existing markers (e.g., 4) a stronger marker will have higher impact on accuracy of the aggregated majority voting. We also observe adding one marker will have linear impact on the acuracy.}
	\label{fig:majority_voting_all}
\end{figure}



Theorem \ref{thm:coverage} discusses that adding more markers makes it more likely to assign weak labels to more samples. 

\begin{theorem} 
	\label{thm:coverage}
	The coverage (probability of voting) \todo{DONE: need to define what we mean by coverage } of majority voting with $K$ markers, with coverages $\{\beta_1, \ldots, \beta_K\}$ is at least as large as the coverage of  most voting marker~$=max_j \beta_j$. 
\end{theorem}

\begin{proof}
	Let $\mathcal{S}$ be the set of all samples and $\mathcal{S}_j$ be the set of samples that are labeled by marker $m_j$. Formally $\mathcal{S}_j = \{s | m_j(s)\neq 0\}$.  Then by definition $\beta_j =p(\mathcal{S}_j )= \frac{|\mathcal{S}_j |}{|\mathcal{S}|}$. Let $\bigcup_j \mathcal{S}_j $ be the set of all weakly labeled samples. Then, the ``effective" coverage of majority voting will be .
	\begin{align}
		\beta &= p(\bigcup_j \mathcal{S}_j ) \nonumber\\
		&= \sum_j p(\mathcal{S}_j ) - \sum_{j_1,j_2}p(\mathcal{S}_{j_1} \cap \mathcal{S}_{j_2})+ \ldots \nonumber\\
		&\qquad+ \sum_{(j_1, \ldots, j_K)} (-1)^{K+1} p(\mathcal{S}_{j_1} \cap \ldots \cap\mathcal{S}_{j_K})\nonumber\\
		&= \sum_j \beta_j  - \sum_{j_1,j_2}\beta_{j_1}  \beta_{j_2}+ \ldots + \sum_{(j_1, \ldots, j_K)} (-1)^{K+1} \beta_{j_1}  \ldots \beta_{j_K}\nonumber\\
		&\geq \max_j \beta_j\nonumber
	\end{align}
\end{proof}


Next, we show that adding a stronger marker $m_{k+1}$ to a set of weaker markers will improve the performance of majority voting more than adding a weak marker.

\begin{proposition} 
	\label{thm:poisson_bonim}
	Let $\{\alpha_1, \ldots, \alpha_k\}$ be the set of accuracies of markers, then a random variable representing the number of correct markers is distributed according to a Poisson Binomial Distribution.
\end{proposition}

Figure  \ref{fig:majority_voting_all} (b) shows how adding a new marker with varying strength to a set of existing  markers will impact the performance of  majority voting. In particular, we observe when the new marker is weaker, and the existing markers are also weak, then the accuracy of majority voting is impacted more negatively compared to when the existing markers are already more accurate.
